Efficient Quantum Lattice Gas Automata

This study presents a novel quantum algorithm for lattice gas automata simulation with a single time step, demonstrating logarithmic complexity in terms of $CX$ gates. The algorithm is composed of three main steps: collision, mapping, and propagation. A computational complexity analysis and a comparison using different error rates and number of shots are provided. Despite the impact of noise, our findings indicate that accurate simulations could be achieved already on current noisy devices. This suggests potential for efficient simulation of classical fluid dynamics using quantum lattice gas automata, conditional on advancements to expand the current method to multiple time steps and state preparation.

==> Mathermatical_description.tex <==

\section{Mathematical description}
The QLGA algorithm consists of a set of particles with different channels, which represent the direction and orientation of the velocity, and a set of lattice points where the particles can be located at a given time $t$. To encode the channels and momentum, we use a system of $n$ qubits forming, forming $N=2^n$ different states.  We can partition the qubits into three subsets: channels, lattice points and ancilla qubits (for computation). The algorithm consists of five steps: initialization, collision, isolation or encoding-swap, shift and measurement. \\

In the first variant of the algorithm, we need $log_2(L)$ qubits for the lattice sites and one qubit per channel, so the total number of qubits is $C+log_2(L)$. For a given time t, we prepare an initial state  $\ket{\psi_0}\equiv\ket{\psi(t-1)}$ using a state preparation operator $I$, which maps a binary state into a quantum representation using an algorithm similar to Mottonen’s \cite{Mottonen_Vartiainen_Bergholm_Salomaa_2005}. At this point, the ancilla qubits are not used, so we omit them in the description. Therefore $\ket{0}^{\otimes n}=\ket{\psi_0}$ and then 

$$I\ket{\psi_0}=\ket{\psi}=\sum\limits_k \alpha_k \ket{C}\otimes \ket{k}$$

 where $\ket{C}$ encodes the occupied channels and $\ket{k}$ represents a superposition over the lattice points. The second step involve only the channel qubits following \hyperref[table_d1q3]{Table 1}, this means that 

$$C_o\ket{\psi}=\sum\limits_k \alpha_k \ket{C'}\otimes \ket{k}$$

where $\ket{C'}$ is the updated state of the channel qubits after the collision step.\\

At this point, a major difference between the two subvariants arises in the way we swap from one encoding to the other. We prepare a superposition not only on the lattice points but also on the particles such that the Hamming weight (or total number of ones) is only one in every state. To create the extra states, ancilla qubits are used. In the subvariant for non-even probabilities, new states are created using Hadamard gates. After that, marked junk states are created to even the probabilities in the superposition (better under noisy conditions). Perhaps a more optimal algorithm for dividing the channels with even probability is possible; nevertheless, this is not a bottleneck due to the small amount of channels compared to lattice sites. For the other subvariant, the sum over ancilla is done for all possible combinations and not only for the particles. To sum up we use an operator $I_s$ (for isolation), such that $I_s$ will be an operation controlled by qubits channels and acting on ancilla. As an example the first subvariant would convert

    $$\ket{011}\longrightarrow \frac{1}{\sqrt{2}}(\ket{01}+\ket{11})$$

while the second 

    $$\ket{011}\longrightarrow \frac{1}{\sqrt{3}}(\ket{011}+\ket{111}+\ket{100})$$

In the first subvariant, we sum over the existing particles using another encoding, as we need fewer qubits. For the second subvariant, we sum over all possible channels in a given lattice site (3), and with a final qubit, we mark if it existed or not (1 if it was present and 0 if not).  To sum up, after the isolation we have

    $$I_s C_o\ket{\psi}=\sum\limits_{k,a} \alpha_{k,a} \ket{C'}\otimes \ket{k}\otimes \ket{a}$$

where a goes over the number of particles for the non-even subvariant (which can be extended to even) and over the number of possible combinations for the even subvariant. An aditional ancilla is used to mark the states which are occupied in the second case $\ket{\psi(t)} = \sum\limits_{k,a} \alpha_{k,a} \ket{C'}\otimes \ket{k}\otimes \ket{a} \otimes \ket{m}$, where m is the marker qubit. \\

The final phase of the algorithm is predicated on the Quantum Fourier Transform (QFT) shift. The objective is to employ shift operators $S^+$ and $S^-$  which translocate particles to the left or right, respectively, such that $S^\pm\ket{k}= \ket{k\pm1}$. The QFT shift algorithm used further optimized this principle. It uses the Fourier transformation ($F$) and phase diagonal multiplication matrix ($P$). TThe qubits on which F is applied are conditioned such that if they are in state 1, the shift opeartor $S^+$ is applied and vice versa for $S^−$, therefore

    $$QFT=F^{-1} P F $$


Additional CNOT gates are used to mark which states are shifted to the right and which to the left. To handle rest particles, extra conditional gates are incorporated in the P layer. If rest particles are present, P is not activated becuase $F^{-1}F=I$. \\

The final step involves measurement and extraction of results for repetition of the process. Theoretically, the general algorithm also includes a swap back from the superposition of particles to the superposition of lattice points to concatenate different time steps, but this aspect is currently under investigation.\\

The algorithm described is general and still works when increasing the dimensions. However, technical challenges arise when performing the shift and managing all the channels in the remaining steps efficiently. As an alternative, we could create special channels to perform the collision step and then recreate these special channels at the end of the time step. In this case, the number of qubits used is $N=log_2(LC)$  These channels encode the states that must be modified under the collision rule, while leaving the rest of the states unchanged.  In this case, the collision follows as
        $$C_o \ket{\psi}= \sum\limits_{k,c_1}\alpha_{k,c_1} \ket{c_1} \otimes \ket{k} + \sum\limits_{k,c_2} \alpha_{k,c_2} \ket{c_2} \otimes \ket{k}$$


where C are the particles which do not suffer any collision and therefore can keep in the same way as before. We can divide $C=c_1+c_2$, and apply the operator on $c_1$ using a control gate.
